PDE-based multi-agent formation control using flatness and backstepping: analysis, design and robot experiments

A PDE-based control concept is developed to deploy a multi-agent system into desired formation profiles. The dynamic model is based on a coupled linear, time-variant parabolic distributed parameter system. By means of a particular coupling structure parameter information can be distributed within the agent continuum. Flatness-based motion planning and feedforward control are combined with a backstepping-based boundary controller to stabilise the distributed parameter system of the tracking error. The tracking controller utilises the required state information from a Luenberger-type state observer. By means of an exogenous system the relocation of formation profiles is achieved. The transfer of the control strategy to a finite-dimensional discrete multi-agent system is obtained by a suitable finite difference discretization of the continuum model, which in addition imposes a leader-follower communication topology. The results are evaluated both in simulation studies and in experiments for a swarm of mobile robots realizing the transition between different stable and unstable formation profiles.

==> figures/concept.tex <==
\begin{tikzpicture}
		\begin{scope}[{->}]
		\draw[line width=0.8pt] (-0.2, 0.0) -- (xyz cs:x=4.2) node[right] {$x^1$};
		\draw[line width=0.8pt] ( 0.0,-0.2) -- (xyz cs:y=4.2) node[above] {$x^2$};
		\end{scope}
		\draw [line width=1.2pt,domain=0:360] plot ({2.5+1.5*cos(\x/2)}, {2.0+1.5*sin(\x)});
		\draw [line width=1.8pt,domain=170:174,->] plot ({2.5+1.5*cos(\x/2)}, {2.0+1.5*sin(\x)});
		\draw (2.9,2.1) node {$ z $};
		
		\foreach \m in {1,...,16}{
			\ifthenelse{\equal{\m}{16}}
			{
				\fill[Green] ({2.5+1.5*cos(\m*360/2/16)},{2.0+1.5*sin(\m*360/16)}) circle (0.1) ;
				\draw ({2.5+1.5*cos(\m*360/2/16)},{2.0+1.5*sin(\m*360/16)}) node[left]{$ \subscr{N} $};
			}
			{
				\fill ({2.5+1.5*cos(\m*360/2/16)},{2.0+1.5*sin(\m*360/16)}) circle (0.1) ;
				
			}
		}
		\draw (2.5,2)+(0: 1.5cm) node[cross=4pt,Green,rotate=10]{};
		\foreach \m in {1,...,4}{
			\draw({2.5+1.5*cos(\m*360/2/16-360/2/16)},{2.0+1.5*sin(\m*360/16-360/16)}) node[above right]{$ \m $};
		}
		\draw ({2.5+1.5*cos(4*360/2/16)},{2.0+1.5*sin(4*360/16)}) node[above]{$ ... $};
		\draw ({2.5+1.5*cos(15*360/2/16)},{2.0+1.5*sin(15*360/16)}) node[left] {$ \subscr{N}-1 $};
		\draw ({2.5+1.5*cos(14*360/2/16)},{2.0+1.5*sin(14*360/16)}) node[left]{$ \subscr{N}-2 $};
		\draw ({2.5+1.5*cos(13*360/2/16)},{2.0+1.5*sin(13*360/16)}) node[below left] {$ ... $};
\end{tikzpicture}
